Safe Perception-Based Control under Stochastic Sensor Uncertainty using Conformal Prediction

We consider perception-based control using state estimates that are obtained from high-dimensional sensor measurements via learning-enabled perception maps. However, these perception maps are not perfect and result in state estimation errors that can lead to unsafe system behavior. Stochastic sensor noise can make matters worse and result in estimation errors that follow unknown distributions. We propose a perception-based control framework that i) quantifies estimation uncertainty of perception maps, and ii) integrates these uncertainty representations into the control design. To do so, we use conformal prediction to compute valid state estimation regions, which are sets that contain the unknown state with high probability. We then devise a sampled-data controller for continuous-time systems based on the notion of measurement robust control barrier functions. Our controller uses idea from self-triggered control and enables us to avoid using stochastic calculus. Our framework is agnostic to the choice of the perception map, independent of the noise distribution, and to the best of our knowledge the first to provide probabilistic safety guarantees in such a setting. We demonstrate the effectiveness of our proposed perception-based controller for a LiDAR-enabled F1/10th car.

==> discreteRobustCBF.tex <==
\section{Discrete measurement-robust control barrier function}\label{sec:CBF}
In this section, we propose the discrete measurement-robust CBF to ensure safety while there exists state estimation error.



\begin{mydef}(Discrete-time measurement-robust control barrier function)
Let $\mathcal{C}\subset\mathcal{D}\subset \mathbb{R}^n$ be the superlevel set of a continuously differentiable function $h: \mathbb{R}^n\rightarrow \mathbb{R}$, then $h$ is
a discrete-time measurement-robust control barrier function (DT-MR-CBF) if there exists $\eta\in[0,1]$ and parameter function pair $(a, b): \mathbb{R}^k\rightarrow \mathbb{R}^2_+$ such that for the control system (\ref{eq:system}):
\begin{align}
    &\mathsf{sup}_{u\in U}[h(f(\hat{x}_t)+g(\hat{x}_t)u_t)-h(\hat{x}_t)\nonumber\\
    &\quad\quad\quad-(a(y)+b(y)||u_t||_2)]\ge -\eta h(\hat{x}_t).
\end{align}
for any $(y, \hat{x})\in V(\mathcal{C})$.
\end{mydef}

Given a DT-MR-CBF $h(x)$, the set consisting of all control values that render $\mathcal{C}$ safe is given by:
\begin{align}
    &K^{dt}_{mrcbf}(y_t, \hat{x}_t)=\{u\in U: h(f(\hat{x}_t)+g(\hat{x}_t)u_t)-h(\hat{x}_t)\nonumber\\
    &\quad\quad\quad\quad-(a(y_t)+b(y_t)||u_t||_2) +\eta h(\hat{x}_t)\ge 0\}
\end{align}



\begin{mythm}\label{thm:nextStateSafety}
 Consider a DT-MR-CBF $h(x)$
defined on $\mathcal{C}\subset\mathcal{D}$. 
Assume that $P(||x_t-\hat{x}_t||_2\le \epsilon')\ge 1-\alpha$ holds for any $x_t\in\mathcal{D}$.
If $h(x)$ is with parameter function pair $(a(y_t), b(y_t))=(\epsilon'(\mathcal{L}_{h}\mathcal{L}_{f}+(1-\eta)\mathcal{L}_{h}), \epsilon'\mathcal{L}_{h}\mathcal{L}_{g})$, 
where $\mathcal{L}_{h}, \mathcal{L}_{f},$ and $ \mathcal{L}_{g}$ are Lipschitz coefficients of $h, f $ and $g$.
Then for any $(y_t, \hat{x}_t)\in V(\mathcal{C})$, any $u(y_t, \hat{x}_t) \in K^{dt}_{mrcbf}(y_t, \hat{x}_t)$ will render $x_{t+1}\in\mathcal{C}$ with probability at least $1-\alpha$, i.e., $P\{h(x_{t+1})\ge 0\}\ge 1-\alpha$.
\end{mythm}
\begin{proof}
See Appendix.
\end{proof}


\begin{remark}
\textcolor{red}{TODO}. Prove the validity of MR-CBF for unicyle model.
\end{remark}

According to Proposition~\ref{prop:bound}, we could directly let 
\begin{align}
    \epsilon'=\underset{i=1, \cdots, N}{\texttt{sup}}R_{x_i, 1-\alpha}+\epsilon,
\end{align}
then the condition $P(||x_t-\hat{x}_t||_2\le \epsilon')\ge 1-\alpha$ in Theorem~\ref{thm:nextStateSafety}  holds naturally.
After we have the next-state safety guarantee, we can derive the trajectory safety guarantee recursively, as shown in the following theorem.
\begin{mythm}\label{thm:trajSafety}
Given $x_0\in \mathcal{C}$, for any $t\in \{0, 1, \cdots, T\}$, $u_t\in K^{dt}_{mrcbf}(y_t, \hat{x}_t)$.
Then we have that the trajectory $x_0x_1\cdots x_T$ is safe with at least probability $(1-\alpha)^T$, i.e., $P\{x_0\in \mathcal{C}, x_1\in \mathcal{C}, \cdots, x_T\in \mathcal{C}\}\ge (1-\alpha)^T$.
\end{mythm}
\begin{proof}
See Appendix.
\end{proof}

\textcolor{red}{Comment/address three issues: 1) how restrictive is (16), i.e., for which systems can we construct valid DT-MR-CBFs, 2) as it's discrete time, it's not computationally easy to solve (16), and 3) how can we obtain the Lipschitz constants. Can we alleviate all three issues with linear barriers? This should be less restrictive if we talk about planning filters.}

Naturally, we can have the following proposition as the solution to the Problem~\ref{problem}.
\begin{mypro}
For any $\theta\in(0, 1)$, let $\alpha=1-\theta^{1/T}$, then the finite time trajectory is safe with probability $\theta$, i.e., $P\{x_0\in \mathcal{C}, x_1\in \mathcal{C}, \cdots, x_T\in \mathcal{C}\}\ge \theta$.
\end{mypro}




% \begin{mythm}
% If we replace $\mathcal{L}_f$ with $\texttt{sup}_{x_t\in[\hat{x}_t-\epsilon(y_t),\hat{x}_t+\epsilon(y_t)]}\frac{df}{dx_t}$, replace $\mathcal{L}_g$ with $\texttt{sup}_{x_t\in[\hat{x}_t-\epsilon(y_t),\hat{x}_t+\epsilon(y_t)]}\frac{dg}{dx_t}$, the above two theorems still hold.
% \end{mythm}

\begin{mylem}
For any $\beta\in\mathbb{R}$, if we let 
\begin{align}
    &K^{dt}_{mrcbf}(y_t, \hat{x}_t)=\{u\in U: h(f(\hat{x}_t)+g(\hat{x}_t)u_t)-h(\hat{x}_t)\nonumber\\
    &\quad\quad\quad\quad-(a(y_t)+b(y_t)||u_t||_2) +\eta h(\hat{x}_t)\ge \beta\},
\end{align}
where $(a(y_t), b(y_t))$ is the same with that in Theorem~\ref{thm:nextStateSafety}. Let $\Bar{h}(x_{t}):=h(x_t)-\frac{\beta}{\eta}$, then we have that:
$P\{\Bar{h}(x_{t+1})\ge 0|\Bar{h}_{x_t}\ge 0\}\ge 1-\alpha$.
\end{mylem}


% \begin{remark}
% It is helpful to reduce conservativeness if we define $\Tilde{h}_{\epsilon(y)}:=\texttt{sup}\{h(x):||x-x^0||_2\le \epsilon(y), \forall x^0\in 
% h^{-1}(\{0\})\}$, and it suffices to have $h(\hat{x})\ge \Tilde{h}_{\epsilon(y)}$. This is less conservative than $\mathcal{L}_h$.
% \end{remark}

% Starting from the above remark, we can have the following proposition. Intuitively, while we have have $|(x_{t+1})-(f(\hat{x}_t)+g(\hat{x}_t)u_t)|\le \epsilon(y_t)(\mathcal{L}_f+\mathcal{L}_g||u_t||_2)$, we do not use $\mathcal{L}_h$ to help bound $h(x_{t+1})$ any more, since it is two conservative; instead, 

% \begin{remark}
% Here, what we assume is $\forall t \in\{1, 2, \cdots, T\}, P\{|x_t-\hat{x}_t|\le \epsilon(y_t)\}\ge 1-\alpha$, and thus we have that $P\{|x_t-\hat{x}_t|\le \epsilon(y_t), \forall t\in \{1, 2, \cdots, T\}\}\ge (1-\alpha)^{T}$.
% However, in~\cite{clark2019control}, they assume that $P\{\texttt{sup}_{t\ge 0}|x_t-\hat{x}_t|\le \epsilon\}\ge (1-\alpha)$, which is a stronger condition.
% \end{remark}
